Shielded Diffusion: Generating Novel and Diverse Images using Sparse Repellency

The adoption of text-to-image diffusion models raises concerns over reliability, drawing scrutiny under the lens of various metrics like calibration, fairness, or compute efficiency. We focus in this work on two issues that arise when deploying these models: a lack of diversity when prompting images, and a tendency to recreate images from the training set. To solve both problems, we propose a method that coaxes the sampled trajectories of pretrained diffusion models to land on images that fall outside of a reference set. We achieve this by adding repellency terms to the diffusion SDE throughout the generation trajectory, which are triggered whenever the path is expected to land too closely to an image in the shielded reference set. Our method is sparse in the sense that these repellency terms are zero and inactive most of the time, and even more so towards the end of the generation trajectory. Our method, named SPELL for sparse repellency, can be used either with a static reference set that contains protected images, or dynamically, by updating the set at each timestep with the expected images concurrently generated within a batch, and with the images of previously generated batches. We show that adding SPELL to popular diffusion models improves their diversity while impacting their FID only marginally, and performs comparatively better than other recent training-free diversity methods. We also demonstrate how SPELL can ensure a shielded generation away from a very large set of protected images by considering all 1.2M images from ImageNet as the protected set.

==> sections/A13_hd_images.tex <==
% Stable Diffusion 3
%git pull; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="a dog plays with a ball" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="A parrot sits in a bench eating some nuts" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="A colorful birthday cake for a kid is being cut open by a knife, revealing its interior. There is a text on top which says ‘Happy Birthday’. Product image for a bakery website." --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="A computer monitor with a futuristic design" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="Circus tent" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="A table layed out with food such as, salad, steamed peas and carrots, steamed corn, and bread rolls" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="stabilityai/stable-diffusion-3-medium-diffusers" --guidance_scale=3 --seed=1 --prompt="Baked pizza with herbs displayed on serving tray at table" --repell_t=500 --repellence_weight=520 --overcompensation=1.6 --timesteps_total=28 --batch_size=1 --number_runs=28

% FLUX
% git pull; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="Baked pizza with herbs displayed on serving tray at table" --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="a dog plays with a ball" --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="A parrot sits in a bench eating some nuts" --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="A colorful birthday cake for a kid is being cut open by a knife, revealing its interior. There is a text on top which says ‘Happy Birthday’. Product image for a bakery website." --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="Circus tent" --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28; python experiments/repellence.py --model="black-forest-labs/FLUX.1-schnell" --guidance_scale=2 --seed=1 --prompt="A table layed out with food such as, salad, steamed peas and carrots, steamed corn, and bread rolls" --repell_t=500 --repellence_weight=630 --overcompensation=1.4 --timesteps_total=28 --batch_size=1 --number_runs=28;


